Advantage of Coherent States in Ring Resonators over Any Quantum Probe Single-Pass Absorption Estimation Strategy

Quantum states of light have been shown to enhance precision in absorption estimation over classical strategies. By exploiting interference and resonant enhancement effects, we show that coherent-state probes in all-pass ring resonators can outperform any quantum probe single-pass strategy even when normalized by the mean input photon number. We also find that under optimal conditions coherent-state probes equal the performance of arbitrarily bright pure single-mode squeezed probes in all-pass ring resonators.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
